Constrained Decision Transformer for Offline Safe Reinforcement Learning

Safe reinforcement learning (RL) trains a constraint satisfaction policy by interacting with the environment. We aim to tackle a more challenging problem: learning a safe policy from an offline dataset. We study the offline safe RL problem from a novel multi-objective optimization perspective and propose the $\epsilon$-reducible concept to characterize problem difficulties. The inherent trade-offs between safety and task performance inspire us to propose the constrained decision transformer (CDT) approach, which can dynamically adjust the trade-offs during deployment. Extensive experiments show the advantages of the proposed method in learning an adaptive, safe, robust, and high-reward policy. CDT outperforms its variants and strong offline safe RL baselines by a large margin with the same hyperparameters across all tasks, while keeping the zero-shot adaptation capability to different constraint thresholds, making our approach more suitable for real-world RL under constraints. The code is available at https://github.com/liuzuxin/OSRL.

==> tables/ablation.tex <==
% \begin{table*}[t]
% \centering
% \renewcommand{\arraystretch}{1.1}
% \resizebox{1.\linewidth}{!}{
% % \begin{tabular}{c|cc|cc|cc|cc|cc}
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
% % \hline
% \toprule
%                           & \multicolumn{2}{c|}{Ant-Run}                                                  & \multicolumn{2}{c|}{Car-Circle}                                               & \multicolumn{2}{c|}{Car-Run}                                                  & \multicolumn{2}{c|}{Drone-Circle}                                             & \multicolumn{2}{c|}{Drone-Run}                                                & \multicolumn{2}{c}{Average}                                                  \\
% \multirow{-2}{*}{Methods} & reward $\uparrow$                                & cost $\downarrow$                                 & reward $\uparrow$                                & cost $\downarrow$                                 & reward $\uparrow$                                & cost $\downarrow$                                 & reward $\uparrow$                                & cost $\downarrow$                                 & reward $\uparrow$                                & cost $\downarrow$                                 & \multicolumn{1}{c}{reward $\uparrow$}            & \multicolumn{1}{c}{cost $\downarrow$}             \\ \hline
% CDT(ours)                 & {\color[HTML]{0000FF} \textbf{89.76}} & {\color[HTML]{0000FF} \textbf{0.83}} & {\color[HTML]{0000FF} \textbf{89.53}} & {\color[HTML]{0000FF} \textbf{0.85}} & \textbf{99.0}                         & \textbf{0.45}                        & {\color[HTML]{0000FF} \textbf{73.01}} & {\color[HTML]{0000FF} \textbf{0.88}} & {\color[HTML]{0000FF} \textbf{63.64}} & {\color[HTML]{0000FF} \textbf{0.58}} & {\color[HTML]{0000FF} \textbf{82.99}} & {\color[HTML]{0000FF} \textbf{0.72}} \\
% CDT(w/o augmentation)     & {\color[HTML]{656565} 93.62}          & {\color[HTML]{656565} 1.53}          & {\color[HTML]{656565} 89.8}           & {\color[HTML]{656565} 1.38}          & {\color[HTML]{656565} 99.58}         & {\color[HTML]{656565} 1.89}          & {\color[HTML]{656565} 74.9}           & {\color[HTML]{656565} 1.35}          & {\color[HTML]{656565} 66.93}          & {\color[HTML]{656565} 1.53}          & {\color[HTML]{656565} 84.97}          & {\color[HTML]{656565} 1.54}          \\
% CDT(w/o entropy)          & \textbf{87.47}                        & \textbf{0.64}                        & {\color[HTML]{656565} 89.94}          & {\color[HTML]{656565} 1.07}          & \textbf{98.92}                       & \textbf{0.44}                        & {\color[HTML]{0000FF} \textbf{73.76}} & {\color[HTML]{0000FF} \textbf{0.97}} & \textbf{62.29}                        & \textbf{0.6}                         & \textbf{82.48}                        & \textbf{0.74}                        \\
% CDT(deterministic)        & {\color[HTML]{656565} 94.21}          & {\color[HTML]{656565} 1.42}          & {\color[HTML]{656565} 89.53}          & {\color[HTML]{656565} 1.43}          & {\color[HTML]{656565} 101.52}        & {\color[HTML]{656565} 17.53}         & \textbf{76.4}                         & \textbf{1.0}                         & {\color[HTML]{656565} 68.44}          & {\color[HTML]{656565} 1.36}          & {\color[HTML]{656565} 86.02}          & {\color[HTML]{656565} 4.55}          \\
% \bottomrule % \hline
% \end{tabular}
% }
% \caption{Evaluation results of the normalized reward and cost. 
% $\uparrow$ / $\downarrow$: the higher/lower, the better.
% Each value is averaged over 20 episodes and 3 seeds.
% \textbf{Bold}: Safe agents whose normalized cost is smaller than 1. 
% {\color[HTML]{656565} Gray}: Unsafe agents.
% {\color[HTML]{0000FF} \textbf{Blue}}: Safe agent with the highest reward.
% }
% \label{tab:ablation}
% \end{table*}

==> tex_files/s9-backup.tex <==
% \textbf{Safe RL.} Constrained optimization techniques are usually adopted to solve safe RL problems~\cite{garcia2015comprehensive, sootla2022saute, yang2021wcsac, flet2022saac}. Lagrangian-based methods use an additional multiplier to penalize objectives with constraint violations. The multiplier can be optimized via gradient descent~\cite{chow2017risk, tessler2018reward} or control-based methods~\cite{stooke2020responsive, chen2021primal}.  Correction-based methods project the unsafe actions into the safe action set, which is also an effective framework for solving safe RL problems. These works incorporate domain knowledge of the target problem to achieve zero violation during safe policy learning~\cite{zhao2021model, luo2021learning}. Another line of work is to perform policy optimization on surrogate policy spaces. 
% CPO utilizes low-order Taylor expansions to approximate the policy space such that the gradient can be solved by convex optimization~\citep{achiam2017constrained}.
% CVPO proposes to improve the policy over a variational distribution and then distill the improvement to a parametrized model~\citep{liu2022constrained}.
% However, ensuring zero constraint violations during training is still a challenging problem.


% Denote $\Tcal \subset \mathcal{T}$ as a set of trajectories, where $\mathcal{T}$ is a family of all the possible trajectories $\{\tau_1, \tau_2,...\}$ that can be collected in the CMDP $\mathcal{M}$.
% We name $\mathcal{T}$ as the full trajectory space (FTS) because it contains all the possible solutions of a safe RL problem, and $\mathcal{T} \subset \mathcal{T}$ as the dataset trajectory space (DTS).
% To characterize the offline dataset $\mathcal{T}$ with both reward and cost metrics, we introduce the Reward Frontier (RF) function that is inspired by the Pareto frontier concept from MOO domain.
% The RF of a dataset $\Tcal$ is denoted by the maximum reward return of trajectories under different cost threshold $\kappa \in \mathbb{C}$, where $\mathbb{C} := \{C(\tau): \tau \in \mathcal{T}\}$ is the set of episodic cost:
% $$\text{RF}(\kappa, \Tcal) = \max_{\tau \in \mathcal{T}} R(\tau), \quad s.t. \quad C(\tau) = \kappa.$$

In this section, we revisit the offline safe RL problem and investigate its taxonomy based on the cost threshold and properties of collected datasets.
Denote $\Tcal = \{\tau_1, \tau_2,...\}$ as a dataset of trajectories.
To characterize the offline dataset $\mathcal{T}$ with both reward and cost metrics, we introduce the Pareto Frontier (PF) and the Reward Frontier (RF) functions that are inspired by the MOO domain.
The PF of a dataset $\Tcal$ with respect to some certain cost threshold $\kappa \in [0,\infty)$ is computed by the maximum reward return of trajectories under constraint $\kappa$:
$$\text{PF}(\kappa, \Tcal) = \max_{\tau \in \mathcal{T}} R(\tau), \quad s.t. \quad C(\tau) \leq \kappa.$$
The RF is defined by the maximum reward with cost $\kappa \in \mathbb{C}$, where $\mathbb{C} := C(\mathcal{T})$ is the set of all the possible episodic cost in $\mathcal{T}$:
$$\text{RF}(\kappa, \Tcal) = \max_{\tau \in \mathcal{T}} R(\tau), \quad s.t. \quad C(\tau) = \kappa.$$
Note that the constraint and the domain of $\kappa$ are different for RF and PF. RF is ``local'', since it represents the highest reward with one certain cost value, which is the most common in the $0$-$1$ cost settings. The definition of RF also indicates that it is not necessarily defined on a continuous space, i.e. it only has definition on $\kappa$, where $\kappa$ is a reachable cost value in dataset $\mathcal{T}$. On the other hand, PF is ``global'', for it is the supremum of all the RF value with respect to a cost smaller than $\kappa$ in dataset $\mathcal{T}$. Another difference from RF is that PF is defined on a continuous $\kappa$ space.
Both functions characterize the shape of the dataset: PF represents the reward upper bound of the trajectories that satisfy the constraint, while RF is the upper bound for the trajectories with corresponding cost returns.
It is also easy to observe that the Pareto frontier $\text{PF}(\kappa, \mathcal{T})$ is a non-deceasing function of $\kappa$, which suggests the trade-offs between safety and task performance: finding a policy with a small cost return usually needs to sacrifice the reward.
It also indicates one important fact: given a target cost return $\kappa$, no policy can achieve more reward than $\text{PF}(\kappa, \mathcal{T})$ without violating the constraint.

Fig.~\ref{fig:cr-plot-dataset} shows an example of the cost-reward return plot of dataset $\mathcal{T}$, each point represents the trajectories with corresponding episodic cost and reward return value. 
The PF curve is shown as the purple curve and the RF points are marked as red.
We observe that the shape of RF and the target cost threshold can characterize the task difficulty.
For example, $\kappa_1$ and $\kappa_2$ in Fig~\ref{fig:cr-plot-dataset} denote two cost thresholds. $(\Tcal, \kappa_1)$ and $(\Tcal, \kappa_2)$ represent two different offline safe RL problems. 
For threshold $\kappa_1$, the maximum reward upon safe trajectories is its RF value $\text{RF}(\kappa_1, \Tcal)$. But for threshold $\kappa_2$, the maximum reward is the PF value and $\text{PF}(\kappa_2, \Tcal)>\text{RF}(\kappa_2, \Tcal)$.
We empirically observe that the latter case is usually easier to solve than the former case, which is not due to $\kappa_2>\kappa_1$, but because the latter case could be \textit{reduced} to an offline RL problem by simply maximizing the reward without considering the cost constraint.  
We describe the latter case as a \textbf{reducible} offline safe RL problem, and conjecture the reducible condition is:

\begin{hypothesis}
 An offline safe RL problem $(\Tcal, \kappa)$ is reducible if and only if: $\text{PF}(\kappa, \Tcal)>\text{RF}(\kappa, \Tcal).$
\end{hypothesis}

This condition indicates that if $(\Tcal, \kappa)$ is reducible, the most rewarding and safe trajectory is with a cost value less than $\kappa$.
We empirically validate the hypothesis by experiments over reducible problems, and find that standard offline RL algorithms can solve the problem well in most cases. 
No constrained optimizations are needed to solve a high-reward and safe policy. The results are shown in Appendix \ref{app:data-reduction}.
The reducible property is related to the temptation definition in the safe RL literature~\cite{liu2022robustness}, which describes the fact that the policy might be tempted during training to achieve high rewards but violate constraints. 
In this work, we are more interested in approximately non-reducible tasks, i.e., for $\forall \kappa \in C(\mathcal{T})$, $\text{PF}(\kappa, \Tcal)\approx\text{RF}(\kappa, \Tcal)$. The rigorous definition of approximately non-reducible by $\epsilon$ non-reducible is presented in Appendix \todo{}. The cost-reward return plots and their RF curves of the datasets in our experiments are also presented in the Appendix~\ref{section: RF curves}.

\begin{figure}[ht]
\vspace*{-2mm}
\centering
\includegraphics[width=0.99\linewidth]{figures/cr-plot.png}
\vspace*{-4mm}
\caption{Cost-reward return plot for a collected dataset. Each point represents trajectories with corresponding episodic cost and reward values in the dataset.}
\label{fig:cr-plot-dataset}

\end{figure}
